CBE Clima Tool: a free and open-source web application for climate analysis tailored to sustainable building design

Buildings that are designed specifically to respond to the local climate can be more comfortable, energy-efficient, and with a lower environmental impact. However, there are many social, cultural, and economic obstacles that might prevent the wide adoption of designing climate-adapted buildings. One of the said obstacles can be removed by enabling practitioners to easily access and analyse local climate data. The CBE Clima Tool (Clima) is a free and open-source web application that offers easy access to publicly available weather files (in EPW format) specifically created for building energy simulation and design. It provides a series of interactive visualization of the variables therein contained and several derived ones. It is aimed at students, educators, and practitioners in the architecture and engineering fields. Since its launch has been consistently recording over 3000 monthly unique users from over 70 countries worldwide, both in professional and educational settings.

==> tables/pmv_ashrae.tex <==
\begin{table}
\centering
\caption{PMV values calculated with the ASHRAE 55–2017 Standard and pythermalcomfort.}
\label{tab:ref_tab_ashrae}
\begin{tabular}{ccccccccc}
\toprule
{} & \multicolumn{6}{c}{Input Data} & ASHRAE & pythermalcomfort \\
{} &   $t_{db}$ & $\overline{t_{r}}$ & $RH$ & $v_{r}$ &  $M$ & $I_{cl}$ &    PMV &              PMV \\
\midrule
0 &       19.6 &               19.6 &   86 &     0.1 &  1.1 &      1.0 &   -0.5 &             -0.5 \\
1 &       23.9 &               23.9 &   66 &     0.1 &  1.1 &      1.0 &    0.5 &              0.5 \\
2 &       25.7 &               25.7 &   15 &     0.1 &  1.1 &      1.0 &    0.5 &              0.5 \\
3 &       21.2 &               21.2 &   20 &     0.1 &  1.1 &      1.0 &   -0.5 &             -0.5 \\
4 &       23.6 &               23.6 &   67 &     0.1 &  1.1 &      0.5 &   -0.5 &             -0.5 \\
5 &       26.8 &               26.8 &   56 &     0.1 &  1.1 &      0.5 &    0.5 &              0.5 \\
6 &       27.9 &               27.9 &   13 &     0.1 &  1.1 &      0.5 &    0.5 &              0.5 \\
7 &       24.7 &               24.7 &   16 &     0.1 &  1.1 &      0.5 &   -0.5 &             -0.5 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/pmv_iso.tex <==
\begin{table}
\centering
\caption{PMV values calculated with the ISO~7730:2005 Standard and pythermalcomfort.}
\label{tab:ref_tab_iso}
\begin{tabular}{ccccccccc}
\toprule
{} & \multicolumn{6}{c}{Input Data} & ISO 7730 & pythermalcomfort \\
{} &   $t_{db}$ & $\overline{t_{r}}$ & $RH$ & $v_{r}$ &  $M$ & $I_{cl}$ &      PMV &              PMV \\
\midrule
0  &       22.0 &               22.0 &   60 &     0.1 &  1.2 &      0.5 &    -0.75 &            -0.75 \\
1  &       27.0 &               27.0 &   60 &     0.1 &  1.2 &      0.5 &     0.77 &             0.77 \\
2  &       27.0 &               27.0 &   60 &     0.3 &  1.2 &      0.5 &     0.44 &             0.43 \\
3  &       23.5 &               25.5 &   60 &     0.1 &  1.2 &      0.5 &    -0.01 &            -0.01 \\
4  &       23.5 &               25.5 &   60 &     0.3 &  1.2 &      0.5 &    -0.55 &            -0.55 \\
5  &       19.0 &               19.0 &   40 &     0.1 &  1.2 &      1.0 &    -0.60 &            -0.60 \\
6  &       23.5 &               23.5 &   40 &     0.1 &  1.2 &      1.0 &     0.50 &             0.36 \\
7  &       23.5 &               23.5 &   40 &     0.3 &  1.2 &      1.0 &     0.12 &             0.12 \\
8  &       23.0 &               21.0 &   40 &     0.1 &  1.2 &      1.0 &     0.05 &             0.05 \\
9  &       23.0 &               21.0 &   40 &     0.3 &  1.2 &      1.0 &    -0.16 &            -0.17 \\
10 &       22.0 &               22.0 &   60 &     0.1 &  1.6 &      0.5 &     0.05 &             0.05 \\
11 &       27.0 &               27.0 &   60 &     0.1 &  1.6 &      0.5 &     1.17 &             1.17 \\
12 &       27.0 &               27.0 &   60 &     0.3 &  1.6 &      0.5 &     0.95 &             0.95 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/set.tex <==
\begin{table}
\centering
\caption{SET values calculated with the ASHRAE~55--2017 Standard and pythermalcomfort.}
\label{tab:ref_tab_set}
\begin{tabular}{cccccccccc}
\toprule
{} & \multicolumn{6}{c}{Input Data} & ASHRAE 55 & pythermalcomfort \\
{} &   $t_{db}$ & $\overline{t_{r}}$ & $RH$ & $v_{r}$ & $M$ & $I_{cl}$ &       SET &              SET \\
\midrule
0  &         25 &                 25 &   10 &    0.15 &   1 &      0.5 &      23.3 &             23.3 \\
1  &          0 &                 25 &   50 &    0.15 &   1 &      0.5 &      12.3 &             12.4 \\
2  &         10 &                 25 &   50 &    0.15 &   1 &      0.5 &      17.0 &             17.0 \\
3  &         15 &                 25 &   50 &    0.15 &   1 &      0.5 &      19.3 &             19.3 \\
4  &         20 &                 25 &   50 &    0.15 &   1 &      0.5 &      21.6 &             21.6 \\
5  &         30 &                 25 &   50 &    0.15 &   1 &      0.5 &      26.4 &             26.4 \\
6  &         40 &                 25 &   50 &    0.15 &   1 &      0.5 &      34.3 &             34.3 \\
7  &         25 &                 25 &   10 &    0.15 &   1 &      0.5 &      23.3 &             23.3 \\
8  &         25 &                 25 &   90 &    0.15 &   1 &      0.5 &      24.9 &             24.9 \\
9  &         25 &                 25 &   50 &    0.10 &   1 &      0.5 &      24.0 &             24.0 \\
10 &         25 &                 25 &   50 &    0.60 &   1 &      0.5 &      21.4 &             21.4 \\
11 &         25 &                 25 &   50 &    1.10 &   1 &      0.5 &      20.3 &             20.4 \\
12 &         25 &                 25 &   50 &    3.00 &   1 &      0.5 &      18.8 &             18.8 \\
\bottomrule
\end{tabular}
\end{table}

